Multi-quark energies in QCD

Four-quark potentials for $SU(2)$ are evaluated in the static limit with the quenched approximation -- using a lattice of $16^3\times 32$ and $\beta=2.4$. The four quarks are restricted to the corners of rectangles with sides upto seven lattice spacings long. The results are analysed in terms of a strategy based on interquark two-body potentials -- as advocated earlier by the authors. This shows that a standard two-body approach overestimates the four-quark binding energy by upto a factor of about three for the largest rectangles.

==> 9209019.2 <==
\renewcommand{\thebibliography}[1]{\section*{REFERENCES\@mkboth
{BIBLIOGRAPHY}{BIBLIOGRAPHY}}\list
{[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
  \advance\leftmargin\labelsep
  \usecounter{enumi}}
  \def\newblock{\hskip .11em plus .33em minus -.07em}
  \sloppy
  \sfcode`\.=1000\relax}

